Towards Optimal VPU Compiler Cost Modeling by using Neural Networks to Infer Hardware Performances

Calculating the most efficient schedule of work in a neural network compiler is a difficult task. There are many parameters to be accounted for that can positively or adversely affect that schedule depending on their configuration - How work is shared between distributed targets, the subdivision of tensors to fit in memory, toggling the enablement of optimizations, etc. Traditionally, neural network compilers determine how to set these values by building a graph of choices and choosing the path with minimal 'cost'. These choices and their corresponding costs are usually determined by an algorithm crafted by engineers with a deep knowledge of the target platform. However, when the amount of options available to a compiler is large, it is very difficult to ensure that these models consistently produce an optimal schedule for all scenarios, whilst still completing compilation in an acceptable timeframe. This paper presents 'VPUNN' - a neural network-based cost model trained on low-level task profiling that consistently outperforms the state-of-the-art cost modeling in Intel's line of VPU processors.

==> sections/VPUNN_06_Checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please read the checklist guidelines carefully for information on how to answer these questions.  For each question, change the default \answerTODO{} to \answerYes{}, \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  For example: \begin{itemize}   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}   \item Did you include the license to the code and datasets? \answerNA{} \end{itemize}
%Please do not modify the questions and only use the provided macros for your answers.  Note that the Checklist section does not count towards the page limit.  In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


  \item For all authors...
        \begin{enumerate}
          \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
                \answerYes{These sections claim novel improvements in VPU compiler scheduling due to the paper and the following sections describe how we achieved this and our results backing up this claim}
          \item Did you describe the limitations of your work?
                \answerYes{Limitations are discussed in Section \ref{limits}}
          \item Did you discuss any potential negative societal impacts of your work?
                \answerNA{This ideas in this paper are purely performance improvements to existing systems}
          \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
                \answerYes{}
        \end{enumerate}
        
        
  \item If you are including theoretical results...
        \begin{enumerate}
          \item Did you state the full set of assumptions of all theoretical results?
                \answerNA{results are not theoretical, but actual gathered from hardware}
          \item Did you include complete proofs of all theoretical results?
                \answerNA{results are not theoretical, but actual gathered from hardware}
        \end{enumerate}
        
        
  \item If you ran experiments...
        \begin{enumerate}
          \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
                \answerNo{Code is proprietary, however we have provided in the appendix a list of the tests used and users of the VPU compiler should be able to observe these performance improvements on these networks}
          \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
                \answerYes{All the training details are specified in Section \ref{hyperparams}}
          \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
                \answerYes{Multiple results of the same experiment can be observed in Figure \ref{experiments_table}}
          \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
                \answerYes{The resources used are specified in Section \ref{hyperparams}}
        \end{enumerate}
        
        
  \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
        \begin{enumerate}
          \item If your work uses existing assets, did you cite the creators?
                \answerNA{This work used performance recordings, compiled by the researchers}
          \item Did you mention the license of the assets?
                \answerNA{The assets used are not available outside of Intel.}
          \item Did you include any new assets either in the supplemental material or as a URL?
                \answerNA{}
          \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
                \answerNA{}
          \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
                \answerNA{}
        \end{enumerate}
        
        
  \item If you used crowdsourcing or conducted research with human subjects...
        \begin{enumerate}
          \item Did you include the full text of instructions given to participants and screenshots, if applicable?
                \answerNA{No human subject research was conducted}
          \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
                \answerNA{}
          \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
                \answerNA{}
        \end{enumerate}
        
        
\end{enumerate}


